Revisiting Driver Anonymity in ORide

Ride Hailing Services (RHS) have become a popular means of transportation, and with its popularity comes the concerns of privacy of riders and drivers. ORide is a privacy-preserving RHS proposed at the USENIX Security Symposium 2017 and uses Somewhat Homomorphic Encryption (SHE). In their protocol, a rider and all drivers in a zone send their encrypted coordinates to the RHS Service Provider (SP) who computes the squared Euclidean distances between them and forwards them to the rider. The rider decrypts these and selects the optimal driver with least Euclidean distance. In this work, we demonstrate a location-harvesting attack where an honest-but-curious rider, making only a single ride request, can determine the exact coordinates of about half the number of responding drivers even when only the distance between the rider and drivers are given. The significance of our attack lies in inferring locations of other drivers in the zone, which are not (supposed to be) revealed to the rider as per the protocol. We validate our attack by running experiments on zones of varying sizes in arbitrarily selected big cities. Our attack is based on enumerating lattice points on a circle of sufficiently small radius and eliminating solutions based on conditions imposed by the application scenario. Finally, we propose a modification to ORide aimed at thwarting our attack and show that this modification provides sufficient driver anonymity while preserving ride matching accuracy.

==> sac arXiv version/abstract.tex <==
\begin{abstract}
	Ride Hailing Services (RHS) have become a popular means of transportation, and with its popularity comes the concerns of privacy of riders and drivers.  ORide is a privacy-preserving RHS proposed at the USENIX Security Symposium 2017 and uses Somewhat Homomorphic Encryption (SHE). % \cite{ORidePaper}.
%At the USENIX Security Symposium 2017, Pham et al. proposed ORide, a privacy-preserving RHS based on Somewhat Homomorphic Encryption (SHE). 
%that provides features such as privacy of riders and drivers, easy payment, accountability, etc.  
%In their protocol, a rider sends her encrypted coordinates to the RHS Service Provider (SP) who then forwards the ride request to drivers in the rider's zone.  Drivers respond back with their encrypted coordinates to the SP. SP homomorphically computes the squared Euclidean distances between the rider and each of the drivers and sends them to the rider.  Rider then decrypts the distances and selects the driver with the shortest distance after which the protocol proceeds with ride establishment.
In their protocol, a rider and all drivers in a zone send their encrypted coordinates to the RHS Service Provider (SP) who computes the squared Euclidean distances between them and forwards them to the rider. The rider decrypts these and selects the optimal driver with least Euclidean distance.
\\
In this work, we demonstrate a location-harvesting attack where an honest-but-curious rider, making only a single ride request, can determine the exact coordinates of about half the number of responding drivers even when only the distance between the rider and drivers are given.
The significance of our attack lies in inferring locations of other drivers in the zone, which are not (supposed to be) revealed to the rider as per the protocol.
%This means that on an average, the rider can identify the location of 1 out of every 2 drivers in the zone. 
%We consider a malicious rider who tries to glean driver location information while trying to solicit rides. 
\\
 We validate our attack by running experiments on zones of varying sizes in arbitrarily selected big cities. Our attack is based on enumerating lattice points on a circle of sufficiently small radius and 
eliminating solutions based on conditions imposed by the application scenario. 
Finally, we propose a modification to ORide aimed at thwarting our attack and show that this modification provides sufficient driver anonymity while preserving ride matching accuracy.
%Finally, we propose and analyze alternate solutions that can be used to fix our attack to preserve location privacy of drivers and discuss the tradeoffs therein.
%Euclidean distance may not always be the most appropriate metric in selecting a driver since  traffic congestion and other road conditions need to be considered as well. 
%Finally, motivated by our attack on the ORide protocol, we propose a simpler, more efficient and accurate solution where the rider can select the time-wise closest driver while providing similar security guarantees as provided by ORide.  Our solution is based on lightweight cryptographic primitives and does not use SHE operations. Compared to ORide, our solution gives a significant reduction in monthly communication bandwidth for both drivers and riders. These reduction factors for a driver and rider are around $\times1000$ and $\times100$, respectively.

\begin{keywords}
	Ride Hailing Services, Privacy and Censorship, Applied Cryptography, Lattice points.
\end{keywords}
\end{abstract}


==> sac arXiv version/conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}
\vspace{-0.1in}
\label{sec:conclusion}
In this paper we present an attack on a privacy-preserving RHS, ORide \cite{ORidePaper}.  We show that an honest-but-curious  rider can determine the coordinates of nearly half the number of drivers in a zone even when only the 
Euclidean distance between the rider and a driver is available to the rider. 
Our attack involves enumeration of lattice points on a circle of appropriate radius and subsequent elimination of lattice points based on geographic conditions.
%For future work, together with the privacy of riders, the location privacy (w.r.t. to riders) of drivers that were not selected
%for a given ride, needs to be considered in Oride. Though in theory one can use a fully homomorphic 
%encryption scheme to achieve this, it is currently inefficient in practice to evaluate circuits that
%need a large multiplicative depth, including sorting of large number of values to
%select the closest rider. It would be interesting
%to explore alternate ways to achieve efficient sorting on private/encrypted data with low multiplicative depth circuits.   
%We intend to extend out attack to other RHS works that improve upon ORide.
%There are recent works that provide efficient solutions, but use partial homomorphic encryption schemes where the security of such cryptosystems need to studied in detail.
%Since many recent works have built upon the basic design of ORide, it will be interesting to explore
%the applicability of our attack to these proposals.
Finally we propose a modification to the ORide protocol as a strategy to mitigate our attack. Here a driver anonymizes her location by choosing a random coordinate within a circle of certain radius around herself. We show through concrete experiments that this technique preserves driver anonymity and accuracy of ride matching.

Although protocols may seem secure in theory, there may arise several complications and vulnerabilities when they are deployed practically, as demonstrated by our attack in Section \ref{sec:cryptanalysis}. In the future it will be interesting to experimentally investigate the notion of driver privacy with respect to both the SP and rider in more recent works following ORide (\textit{lpRide}, \cite{lpRideYu}, \textit{pRide} \cite{pRideLuo}).
\vspace{-0.1in}
\subsubsection*{Acknowledgements.}
The authors would like to thank Sonata Software Limited, Bengaluru, India for funding this work.  
We also
thank the anonymous reviewers of ACM CCS2020, USENIX Security 2021 and SAC 2021 for their
valuable comments and suggestions.


==> sac arXiv version/cryptanalysis.tex <==
\section{Analysis of ORide Protocol}
\label{sec:cryptanalysis}
In this section we briefly recall the ORide protocol of  \cite{ORidePaper}, followed by a security analysis of the protocol at the rider's end.
We then describe our attack that would allow a rider to predict a driver's location with good accuracy, and present the results of practical experiments. 

\subsection{ORide : A Privacy-Preserving Ride Hailing Service}

\label{oride_intro}

As mentioned in Section \ref{sec:introduction}, ORide is a privacy-preserving ride hailing service
%was published at the 26th USENIX Security Symposium \cite{USENIX17}.  
that uses an SHE scheme to match riders with drivers. 
In the process, identities and locations of drivers and riders are not revealed to the SP.  
The protocol provides accountability for SP and law-enforcement agencies in case of a malicious driver or rider.  
It also supports convenience features like automatic payment and reputation-rating of drivers/riders.  
In short, it is a complete and practical solution along with novel methods  that help keep the identity of drivers and riders oblivious to the SP, together with accountability and convenience.
The experiments done in their paper use real datasets consisting of taxi rides in New York city \cite{OrideNYCDataset}. 
Their instantiation provides 112-bit security, based on the FV SHE scheme \cite{EPRINT:FanVer12} which relies on the hardness of the Ring Learning With Errors (RLWE) problem. 

%\paragraph{Na\"{i}ve approach}
%The plaintexts and ciphertexts in the FV scheme are elements of integer polynomial quotient rings. 
%These polynomials have $d$ coefficients, and $d$ was set to 4096 in order to achieve 112-bit security. 
%A na\"{i}ve approach would be for the rider to encrypt her planar coordinates and send this (along with her public key and zone of pick-up location) to SP. 
%The SP forwards the rider's public key to every driver in the rider's zone. 
%Each driver encrypts her (integer) planar coordinates using the rider's public key, and sends this to SP. 
%If there are $n$ drivers in this zone, SP now has $n$ encrypted polynomials.
%SP homomorphically computes the (encrypted) squared Euclidean distance  between the rider and each driver separately, and sends these $n$ resultant ciphertexts back to the rider, who can decrypt and choose the closest driver based on the Euclidean distance.

%\paragraph{Optimizations}
%ORide proposed two optimizations over the na\"{i}ve approach: ciphertext packing and transform processing. 
%In ciphertext packing, a driver $D_i$ in the zone encrypts her coordinates into the $i$\textsuperscript{th} coefficient of the polynomial. 
%%(ORide shows that $d \geq n$, and so this is indeed possible).
%The SP aggregates all received ciphertexts into a \textit{single} polynomial, where coefficient $i$ contains coordinates of $D_i$. 
%This would mean that each homomorphic operation affects all coefficients in parallel.
%Hence, the SP can finally send just one ciphertext whose $i$\textsuperscript{th} coefficient contains the squared Euclidean distance between the rider and the driver $D_i$, thereby saving bandwidth and processing time in decryption.
%Coefficient-wise multiplication in these polynomials is necessary when computing Euclidean distances. 
%Whereas polynomial addition and subtraction is easy to perform coefficient-wise, polynomial multiplication leads to a convolution product of the coefficients.
%Hence, the second optimization --- the Number-Theoretic Transform (NTT) is used to transform convolution products into coefficient-wise products (and vice-versa). 

%\subsubsection{ORide protocol}
 
We give below a high-level overview of the ORide protocol relevant to our attack.
(For more details, the reader is referred to the original paper).
%\begin{figure}[htpb]
%%\vspace{-1cm}
%\includegraphics[height=4.1in, width=220pt]{../img/ORide-original.png}
%%\vspace{-.7in}
%\caption{The ORide protocol} \label{fig:oride-original}
%%\vspace{-1cm}
%\end{figure}
%\begin{itemize}
%\item Drivers who wish to provide their services register with the SP using an app on their smartphones. 
%On registration, the SP provides drivers with  anonymous credentials---deposit tokens to be used during their communications with itself and digital signatures for communication with riders.  
The registered drivers periodically advertise their geographical zones to the SP.  
These zones are predefined by the SP and available to drivers and riders. The size of a zone
is chosen in such a way that there are sufficiently many riders and drivers to ensure
anonymity while maintaining the efficiency of ride-matching.
 When a rider wishes to hail a ride, she generates an ephemeral FV public/private key-pair $(p_k, s_k)$. 
She encrypts her planar coordinates using this key and sends it to the SP along with $p_k$ and her zone $\mathcal{Z}$.
SP broadcasts the public key $p_k$ received from the rider to each driver in $\mathcal{Z}$.
The $i$\textsuperscript{th} driver $D_i$ encrypts her planar coordinates using $p_k$ and sends it to SP.
SP homomorphically computes the squared values of the Euclidean distances between each driver and the rider in parallel, and sends the encrypted result to the rider. 
The rider decrypts the ciphertext sent by SP to obtain the squared Euclidean distance to each driver $D_i$. 
She then selects the driver with smallest squared Euclidean distance and then notifies the SP of the selected driver. 
This selected driver is in turn notified by the SP. 
As part of the ride establishment protocol a secure channel is then established between the rider and the driver. They then proceed to service the ride request as per the protocol. Further steps, although important, are not relevant to our work and, hence, we do not mention them here.
%\end{itemize}

\subsection{ORide : Threat Model}

\label{oride_threat_model}

%\textit{Assumptions in ORide.}
The threat model considered in ORide is that of an honest-but-curious SP, whereas the drivers and riders are active adversaries who do not collude with the SP.    We consider the same adversarial model in this paper as well.
%They assume that the drivers and riders do not collude with the SP.
All the plaintext information is encoded as integer polynomials before encrypting with the  FV SHE scheme.
%s operate on finite rings, all plaintexts must be input as integers.
In ORide, the apps on the drivers and riders use a map-projection system such as UTM \cite{UTMGrid} to 
convert pairs of floating-point latitudes and longitudes to planar integer coordinates.  
%In such systems, the great-circle distance (in metres) between latitude-longitude coordinates over the earth corresponds to the Euclidean distance between planar UTM coordinates.  
Drivers use third-party services like Google Maps or TomTom for navigation.


\subsection{Attack: Predicting Driver Locations}

\label{analysis}

\begin{algorithm}[h!]
\small
\SetAlgoLined\DontPrintSemicolon

\SetKwFunction{algoOne}{Predict_Driver}
\SetKwProg{myalgoOne}{Procedure}{ : }{}

\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{ The rider's zone $\mathcal{Z}$, number of drivers $n$ inside $\mathcal{Z}$, rider's coordinates $(X_r, Y_r)$, Euclidean distances $d_i$ between the rider and driver $D_i$ ($\forall i=1,\cdots ,n$)}
\Output{ For each driver $D_i$, $\mathcal{S}'_{i}$ denotes the prediction set made for the location of $D_i$ by the rider}

\myalgoOne{\algoOne{$\mathcal{Z}, n, (X_r, Y_r), \{d_i\}_{i=1}^{n}$}} {

\vspace{5pt}

$avg = 0$;  %% We say this at the bottom \MyComment{Average number of predicted locations for a driver} \\
$exact = 0$ %% We say this at the bottom \MyComment{Percentage of times a driver was predicted exactly} \\


\For{\textnormal{each driver} $D_{i}$}{
%\MyComment{$d_i$ : Euclidean distance between (rider, $D_i$)} \\
\textbf{Receive}: $d_i$ from SP \\

$\mathcal{S}_i = \phi$ \MyComment{Store unique lattice points}\\
	\For{$x = 0$ \KwTo $\lfloor \sqrt{d_i} \rfloor$}{
	$y = \sqrt{d_i - x^2}$ \\
%	\MyComment{Check if $y$ is also an integer} \\
	\If{$y$ is an integer} { 
%			 \MyComment{If $y$ is an integer, collect the possible symmetric values for $x$ and $y$} \\
		 $T = \{\ (x, y), (-x, y), (-x, -y),(x, -y),$\\\hfill $(y, x), (-y, x), (-y, -x), (y, -x) \ \}$ \\
		 \For{$(x', y') \in T$}{
			\MyComment{Compute predicted location for $D_i$} \\
			$X_d = X_r + x'$; 
			$Y_d = Y_r + y'$ \\
			\If{($X_d, Y_d$)\textnormal{ is inside $\mathcal{Z}$}}{
		$\mathcal{S}_i \coloneqq \mathcal{S}_i \cup \{\ (x, y)\ \}$
		}
		 }			 
	}
	}
$\mathcal{S}'_i = \phi$  \MyComment{Filtered lattice points on road} \\
	\For{$(X_d, Y_d) \in \mathcal{S}_i$}{
	\MyComment{Use Google Maps  API to check if the coordinates lie on road} \\
	${(x, y)}_{road} = \mathsf{RoadAPI}(\ (X_d, Y_d) \ )$ \\ \vspace{5pt}
	\If {$\textnormal{distance between } (X_d, Y_d) \textnormal{ and } {(x,y)}_{road} <= 3 \textnormal{ metres }$ }{

	\vspace{3pt}
	$\mathcal{S}'_i \coloneqq \mathcal{S}'_i \cup \{\ (X_d, Y_d)\ \}$
	}
	}
\MyComment{$\|\mathcal{S}'_i\|$ is the number of locations that the rider has predicted for $D_i$} \\
$avg \coloneqq avg + \|\mathcal{S}'_i\|$ \\
\If{$\|\mathcal{S}'_i\|\ == 1$}{
	$exact += 1$ 	\MyComment{Exact driver loc predictions} \\
	}
%\textbf{Output}: $ \mathcal{S}'_i $ \MyComment{Predicted locations for $D_i$} \\
}
$avg \coloneqq avg \ / \ n$;\  %\MyComment{Average over $n$} \\
$exact \coloneqq exact \ / n \times 100$ \\ %\MyComment{Percentage over $n$} \\
%\textbf{Output}: $avg$  \\
\textbf{Output}: $exact$, $avg$, $ \mathcal{S}'_i $ 
%\MyComment{Percentage of times a driver was predicted exactly} \\
}

\caption{Location-harvesting Attack on ORide}
\label{algo:cryptanalysis}
\end{algorithm}



We now analyze the ORide protocol from the rider's end. 
For ease of explanation, the rest of our paper shall refer to the squared Euclidean distance between two 
points as simply the Euclidean distance. 
In the ORide protocol, before a rider finally chooses the closest driver, she is given a list of Euclidean 
distances corresponding to drivers in her zone.
In this case, the rider only gets to know the Euclidean distance to each driver, and not the driver's exact coordinates. 
Mathematically, this would mean that there are infinite possibilities for the driver's location on the 
circumference of a circle defined from the rider's perspective. 
%We would like to note that there is no explicit analysis of the privacy (w.r.t. riders) of the drivers who responded to a ride request but were not selected for the ride. As we shall see in Section \ref{sec:solution}, if this aspect of the privacy of the drivers is ignored, then a more efficient protocol exists.

On the contrary, we % we use live map and traffic data using Google Maps API \cite{googleroadapi} to 
show that the driver's Euclidean distance allows the rider to identify the actual location of a driver with good probability.
We show that by identifying road networks on a live map (using Google Maps API \cite{googleroadapi}), along with the fact that ORide uses integer 
coordinates, the number of possible driver locations from the rider's perspective can be reduced 
significantly, to around $2$ locations on average. 
%Therefore the probability with which a rider correctly identifies the driver's location is $\frac{1}{2.1} \times 100 \approx 48\%$.

\textit{Remark}. 
While we make use of the fact that ORide uses integers coordinates, our attack would also work for fixed-
point encoding of the coordinates. This is because the current (exact) techniques for fixed-point 
encodings for RLWE-based SHE schemes essentially use the scaled-integer representation \cite{SAC:CSVW16}. %Our attack also naturally carries over even if the SP uses the $p$-norm metric in the ORide protocol instead of the Euclidean distance (refer to Section \ref{sec:p-norm}).
%, and hence is independent of how the coordinates are encoded.
%\end{remark}

Before we proceed with our analysis, we make the assumption that when the rider requests a ride and when 
each driver in the zone sends her encrypted coordinates to SP, the drivers are on road (since we use Google Maps API in our experiments, these include city roads, parking lot roads and many other categories, as specified by the definition of a \emph{road segment} by Google Maps \cite{googleroadapi}).
This assumption is reasonable since a vast majority of the active drivers at any point in time constantly move around the city looking for potential rides or about to finish serving another ride.

When we say that a driver's coordinates lie on road, we mean that the coordinates lie within the borders 
of the road. The current standards for lane width in the United States recommends that each lane is 3 metres wide on average \cite{roadwidth}. Since many roads within a city consist of 2 lanes, we assume that a pair of coordinates lie on road if the location is within 3 metres from the centre of a road (neighborhoods in many cities around the world consist mostly of 2 lane roads, so our experiments give a fairly accurate idea of location recovery probabilities). We stress that the drivers can be anywhere in the zone on any road and our experiments indeed follow this distribution.

\textit{Rider's attack.}
A rider performs the following attack to obtain a set of possible locations for a driver. At the time of ride request, let the rider coordinates be $(X_r, Y_r)$ and the driver coordinates be $(X_d, Y_d)$, which the rider does not know. Let the rider's zone be denoted by $\mathcal{Z}$. SP receives the encrypted values of $X_r, X_d, Y_r, Y_d$, then homomorphically computes the Euclidean distance in encrypted form, and the rider decrypts this to obtain $N = (X_r-X_d)^2 + (Y_r-Y_d)^2 $.
%(As a remark, the value of $n$ depends on the size of the predefined zone. If the zone is bigger in size, then  a driver inside the zone could be further away from the rider, resulting in a larger possible value of $n$).
If $N$ is not too large (refer to Section \ref{practical_implementation} for a concrete discussion on bounds for $N$), the rider can efficiently find all integer solutions to the equation $x^2 + y^2 = N$. 
The rider could use an $O(\sqrt{N}~)$ algorithm to accomplish this: keep a solution-set, and for every 
integer $x' \in [0, \lfloor{\sqrt{N}}~\rfloor]$, compute $y' = (N - x'{}^{2})^{1/2}$. 
If $y'$ is an integer, add the coordinates $(x', y')$, $ (x', -y')$, $  (-x', y')$, $  (-x', -y')$, $  (y', x')$, $  (y', -x')$, $  (-y', x')$ and $(-y', -x') $ into this set. 
%This is the best algorithm we are aware of to enumerate the lattice points. 
%If the factors of $N$ are provided, then it may be possible to do it in time $\tilde{O}(\sqrt{P}~)$, where $P$ is the largest prime factor dividing $N$ (see Section \ref{sec:large_values}). 

Now, rider maintains a set $\mathcal{S}$ containing the possible driver locations. For each integral solution $x_i, y_i$ satisfying $x_i^2+y_i^2=N$, the rider identifies potential driver coordinates as 
$ (X'_{d, i} = X_r + x_i, Y'_{d, i} = Y_r + y_i)$
and adds $(X'_{d, i}\,, Y'_{d, i})$ to $\mathcal{S}$ if $(X'_{d, i}\,, Y'_{d, i})$ is inside $\mathcal{Z}$.

%Note that there always exist $X'_{d, j}$ and $Y'_{d, j}$ such that $X_d = X'_{d, j}$ and $Y_d = Y'_{d, j}$. In other words, even though the rider does not know the driver's coordinates, they are one among the solutions obtained by the rider, since the driver's coordinates satisfy \eqref{eq1}.

Once the rider obtains these possible driver coordinates in $\mathcal{S}$, she checks whether each solution lies on road. (Google Maps Road API \cite{googleroadapi} can be used to achieve this). 
%(As remarked earlier in this subsection, given a coordinate, the rider determines her distance from the center of the road closest to it using Road API; if this distance is less than 3 metres, the coordinates lie on road).
The rider now obtains a filtered set of coordinates $\mathcal{S^'} \subseteq \mathcal{S}$ that are inside $\mathcal{Z}$, and also lie on a road. 
Note that since the actual coordinates of the driver also satisfy these conditions, it is \emph{always} present in this set.
The cardinality of $\mathcal{S}'$ would denote the number of predicted locations for a driver. If this cardinality is exactly one, then the rider has successfully predicted the driver's exact location.
Our  attack is summarized in Algorithm \ref{algo:cryptanalysis}.   
The algorithm takes as input the Euclidean distances of drivers in the zone and, for each driver, outputs the set 
of filtered coordinates $\mathcal{S}'$.  It outputs the number of predicted locations \textit{avg}, averaged over all drivers.  Finally, it outputs \textit{exact}
which denotes the number of drivers for whom exactly one location is predicted.

We present an illustrative example in Figure \ref{fig:map-example}. Consider a large zone in Dallas, USA, with a cartesian grid embedded over the road view of the map. Consider a driver and a rider pair inside this zone. The rider is said to be located at the origin, and let the driver be at coordinates $ (4,3) $ (which agrees with our assumption that drivers lie on road). The rider is given the Euclidean distance $ 25 $ to this driver. She then obtains all lattice points lying on this circle: $ \mathcal{S} = \{ (\pm 3, \pm 4), (\pm 4, \pm 3), (\pm 5, 0), (0, \pm 5) \} $. Out of these, the rider filters out coordinates that lie on road (shown as green dots in Figure \ref{fig:map-example}) to obtain $ \mathcal{S'} = \{ (-4, 3), (4, 3), (5, 0), (0, -5) \} $. Note that the driver's actual coordinates belong to $ \mathcal{S'}$. Note also that if the rider's location, her zone and the Euclidean distance to this driver was given as input to Algorithm \ref{algo:cryptanalysis}, we would receive as outputs $ \mathcal{S}' = \{ (-4, 3), (4, 3), (5, 0), (0, -5) \}, avg = 4, exact = 0 $.

\begin{figure}
%\vspace{-1cm}
\centering
\includegraphics[,width=220pt]{new-map}
%\vspace{-.7in}
\caption{Illustrative example of location prediction of a single driver by a rider.} \label{fig:map-example}
%\vspace{-1cm}
\end{figure}

\textit{Remark}.
In the scenario of ORide, the rider's zone usually consists of multiple drivers. 
Note that in Algorithm \ref{algo:cryptanalysis}, when calculating the possible coordinates $\mathcal{S}'_i$ for the $i$\textsuperscript{th} driver $D_i$, the analysis that a rider performs for one driver is \emph{independent} of the analysis for other drivers. 
Therefore, the averaged results for multiple drivers in one execution of the attack 
(if the driver locations are randomly and independently sampled subject to above conditions)
is equivalent to the averaged results over multiple executions of the attack in the case of only a  
single driver present inside the zone.

Our implementation of the attack will therefore consider one driver inside the zone, and average the results over multiple experiments, considering randomly chosen rider and driver locations each time. 

\subsection{Implementation of Our Attack}

\label{practical_implementation}

Using Google Maps API for Python \cite{googleroadapi_python}, we performed experiments to validate our attack across four arbitrarily chosen cities: New York city, Dallas, Los Angeles and London %\footnote{The code for our attack presented in Section \ref{sec:cryptanalysis} can be accessed at \href{https://pastebin.com/q8dZiLCq}{https://pastebin.com/q8dZiLCq}}
\footnote{The code for our attack presented in Section \ref{sec:cryptanalysis} can be accessed at \href{https://github.com/deepakkavoor/rhs-attack}{https://github.com/deepakkavoor/rhs-attack}}.
%We have submitted the code for our attack as auxiliary material with this submission, and it will be made available publicly after acceptance.
We ran our experiments over zones of sizes $A = $ \{ 1 km\textsuperscript{2}, 4 km\textsuperscript{2}, 9 km\textsuperscript{2}, 25 km\textsuperscript{2}, 100 km\textsuperscript{2}, 400 km\textsuperscript{2}, 900 km\textsuperscript{2} \} (with the exception of New York city due to its geography having multiple smaller discontinguous areas). 
%The results are tabulated in Table \ref{tab1}.
For each city, and for each zone size $a \in A$, we performed 30 experiments. In each experiment, a random square zone $\mathcal{Z}_a$ of area equal to $a$, was chosen.
We chose a random latitude-longitude pair inside $\mathcal{Z}_a$ for the rider in this zone. 
For a driver, we similarly chose a random latitude-longitude pair inside $\mathcal{Z}_{a}$ that was on road (Google Maps Road API was used to accomplish this).

These coordinates were converted to UTM coordinates using the \emph{utm} library for Python \cite{utmPython}.
The Euclidean distance between these UTM coordinates was made available to the rider.
Finally, we obtained the driver's filtered set of probable locations as described in Algorithm \ref{algo:cryptanalysis}. After obtaining the predicted driver coordinates, we averaged the number of such predicted locations over multiple experiments. We also counted the percentage of experiments in which the rider predicted exactly one location. 
With these considerations, our results for varying grid sizes and cities are shown in Table \ref{tab1}. 

\begin{table*}
	\small
	\renewcommand{\arraystretch}{1.3}
	%\hspace{-1.3cm}
	\caption{The rider's prediction based on Algorithm \ref{algo:cryptanalysis}, averaged over 30 experiments.}
	\label{tab1}
	\centering
	\renewcommand*{\arraystretch}{1.1}
	\begin{tabular}{c|c c c c|c c c c}
%	\begin{tabular}{ c|  >{\centering\arraybackslash}m{30pt} >{\centering\arraybackslash}m{30pt}  >{\centering\arraybackslash}m{40pt} >{\centering\arraybackslash}m{30pt}|  >{\centering\arraybackslash}m{30pt} >{\centering\arraybackslash}m{30pt}  >{\centering\arraybackslash}m{40pt} >{\centering\arraybackslash}c  }
%		\hline
		Zone Size& 
		\multicolumn{4}{p{5cm}}{\centering Number of possible driver locations \\ (Output $avg$ of Algorithm \ref{algo:cryptanalysis})} &
		\multicolumn{4}{|p{5cm}}{\centering Exact driver locations prediction \\ (Output $exact$ of Algorithm \ref{algo:cryptanalysis})} \\[0.2em]
		\cline{2-9}
		(km\textsuperscript{2}) & New York & Dallas & Los Angeles & London & New York & Dallas & Los Angeles & London  \\
		\hline 
		1   & 2.6 & 1.8 & 2.5 & 1.6 & 32\% & 52\% & 32\% & 60\% \\
		2   & 2.4 & 1.6 & 2.1 & 1.6 & 48\% & 52\% & 36\% & 68\% \\
		4   & 2.0 & 2.0 & 1.8 & 1.7 & 44\% & 44\% & 52\% & 56\% \\
		9   & 2.7 & 1.9 & 2.1 & 2.3 & 38\% & 56\% & 48\% & 40\% \\
		25  & 2.6 & 2.2 & 2.4 & 2.1 & 36\% & 44\% & 36\% & 48\% \\
		100 & 2.7 & 2.1 & 2.2 & 1.8 & 32\% & 44\% & 44\% & 56\% \\
		400 & 2.3 & 2.1 & 2.5 & 1.8 & 36\% & 48\% & 28\% & 56\% \\
		900 &  -- & 2.8 & 3.1 & 2.4 &  --  & 40\% & 24\% & 40\% \\
%		\hline
	\end{tabular}
\end{table*}

\subsubsection{Timings} 
Our experiments were performed on an Intel Core i5-8250U CPU @ 1.60 GHz with 8 GB RAM running Ubuntu 18.04.4 LTS.
On an average, one experiment (as described above) took 2 seconds for each driver, showing that our attack is indeed efficient, thus allowing a rider to practically obtain any driver's coordinates with good confidence.

\subsubsection{Interpretation of values in Table \ref{tab1}}
Our experiments showed that the average number of solutions to $x^2+y^2=N$  over all the aforementioned zone sizes was 20. When we filter these solutions based on whether they lie inside a zone and on road, the average possible driver coordinates were 2 in number (as indicated by the value \emph{avg} in Table \ref{tab1}), which is a significant reduction. Although it may seem that Euclidean distance gives fair anonymity to driver coordinates, our attack shows that in practice, this is not the case, and a rider can indeed find the driver's location with good probability. 
We also note from the average value of \emph{exact} in Table \ref{tab1} that the rider can predict the driver's exact location around 45\% of the times.

Note that in each city, as zones get bigger, the number of lattice solutions and filtered coordinates tend to increase leading to higher \emph{avg}. More lattice solutions imply that the event when a rider predicts exactly one location for a driver is rare, thus decreasing the value of \emph{exact}. This trend can be verified from  Table \ref{tab1}.

%We also observed that the average number of predicted locations in London were less compared to other cities. We reason that due to narrower roads in London (cite?), the probability that a random driver coordinate lies within 3 metres of a road is low, resulting in lesser number of predicted locations for a driver. This also implies that probability of predicting exactly one location is higher, which is apparent from the larger values of \emph{exact} in London.

\subsubsection{Anonymity Sets}

In ORide, when the rider makes a request, she sends her zone identity to SP, and the SP now knows which zone the rider is in. 
This zone could contain the rider's home/work address. 
As pointed out in the ORide paper \cite{ORidePaper}, SP might be able to guess the identities of the riders if this pick-up zone had a limited number of ride activities, and a limited number of riders (as an extreme example, a zone where only one rider lives).
Therefore, ORide defines zones in such a way that each zone has at least a large minimum number of ride requests per day. 
This large minimum is referred to by them as the \emph{anonymity-set} size.
The choice of size of these zones is left to the SP, based on balancing the communication bandwidth requirements and sizes of anonymity sets in those zones.
(A very high anonymity set would mean that the demand for rides in that zone is high, leading to longer ride matching times and higher bandwidth usage).

We justify our choice of choosing zones of sizes $a \in A$ for our experiments:
\begin{compactlist}

\item In a densely populated city like New York City (population density\footnote{\href{https://worldpopulationreview.com/us-cities}{https://worldpopulationreview.com/us-cities}} 11,084 persons/km\textsuperscript{2}), where more people tend to use ride hailing services, a smaller zone size would suffice to achieve the required anonymity-set size.
In a sparse city like Dallas (population density 1,590 persons/km\textsuperscript{2}), where fewer ride-hailing activities occur, these zones would have to be bigger in size to achieve the same anonymity for riders.
%We wanted our experiments to run over different possible sizes of zones, so that no matter what demarcation of zones is chosen by the SP, our results would be reliable in all such cases. 
%By choosing variations between densely populated and sparse cities, we have thus obtained these results from a broader perspective.
Taking into consideration the different possible zone sizes in both densely populated and sparse cities, the experiments validate our attack in zones of areas ranging from 1~km\textsuperscript{2} to 900~km\textsuperscript{2}.

\item We analyzed the NYC Uber-Dataset \cite{NYCDataset} for May 2019, and deduced that the demand for taxi rides was very high in Manhattan compared to the other boroughs of NYC. We chose May since this month had one of the highest ride requests for Uber in 2019.
Based on this, we followed the zone demarcation that was proposed by ORide: each Census Tract (CT) \cite{NYCensusTract} in Manhattan is considered as one zone. The boroughs of Queens and Bronx are merged into one zone, and the boroughs of Brooklyn and Staten Island are merged into one zone.
The size of each CT in Manhattan varies between 1 km\textsuperscript{2} and 4 km\textsuperscript{2} that correspond to zone size of higher activity.  Since the boroughs other than Manhattan have lesser activity, these zones are expected to have a larger area. Indeed, the combined area of Queens and Bronx is around 390 km\textsuperscript{2}, and the combined area of Brooklyn and Staten Island is around 330 km\textsuperscript{2}. Since this is the primary zone demarcation proposed by the authors of ORide, we found it reasonable to include these ranges of areas for our experiments in Table \ref{tab1}.

\end{compactlist}

We next discuss few details involved in the implementation of our attack.
\begin{compactlist}
\item  Although zones can be of any geographical shape, we chose square zones for ease of choosing 
random coordinates inside its boundary, and to simplify checking whether a given coordinate lies inside the zone.
%We stress that except for this ease of code implementation, our analysis never depended on the fact that zones are square in shape: the solutions to \eqref{eq1} would be exactly the same, and the filtering based on whether drivers are present inside the zone and lie on road, would be identical as well. 
%Hence, our results are similar for any such geographical demarcation of zones.

\item Latitude-longitude coordinates were converted into UTM formats using the \emph{utm} library for Python. 
On an average, this conversion  results in a difference of 0.5 metres between the original coordinate and the planar coordinate's representation.
%Precisely, upon converting a latitude-longitude coordinate $P_{latlon}$ into UTM format $P_{utm}$, and converting $P_{utm}$ back into its latitude-longitude representation $P'_{latlon}$, the two locations $P_{latlon}$ and $P'_{latlon}$ were just 0.5 metres apart on average. 
For all practical purposes, this difference is very small, and the two coordinates can be considered to represent the same location.

\item As discussed earlier, based on the NYC Uber-Dataset and ORide's proposed demarcation, even large sparse zones that have a sufficiently big anonymity-set would rarely exceed $30\times 30=900$ km\textsuperscript{2}. 
Note that the Euclidean distance between two UTM coordinates is equal to the distance (in metres) between latitude-longitude representation of those points. 
Hence, the maximum value of $N$ for a $d \times d$ grid would be $2d^2$.  For a 
30 km $\times$ 30 km grid, $d$ would be $30,000$.  
Since there exists an $O(\sqrt{N}) = O(d)$ algorithm to compute solutions to $x^2+y^2=N$, it is indeed feasible for the rider to perform this analysis on modern computers in very less time, even for different zone structures chosen by SP.  
%For asymptotically large values of $N$ we provide an overview of the behaviour of our attack in Section \ref{sec:large_values}. 

%\item  The width of a lane was chosen to be 3 metres in our experiments (based on the recommendation in \cite{roadwidth}) and it was assumed that most of the roads under consideration are 2 lanes wide. We stress that neighbourhoods in many cities around the world consist majorly of 2 lane roads, and so our experiments give a fairly accurate idea of location recovery probabilities.
%However, in practice, roads could be wider than this. Suppose we choose all roads to consist of 4 lanes (though this is not reasonable), implying that every road is 12 metres wide. Now in Algorithm \ref{algo:cryptanalysis}, for every $(X_d, Y_d) \in \mathcal{S}_i$, we would check if it is 6 metres away from road. Compared to the case of 2 lane roads, there is a slightly greater chance that our automated attack classifies this candidate solution to lie on a road, and the size of $\mathcal{S}'_i$ would be bigger in such cases. 
%
%For the scenario of wide roads, sometimes this automation may lead to misclassification as well, since a point that was 6 metres away from a very narrow 2 lane road (of half width 3  metres) would be misclassified to lie on road.
%%The size of $\mathcal{S}'_i$ would be bigger in such cases. 
%In such scenarios, instead of automating this process using Google Maps Road API, the rider could manually check whether these points lie on road (using Satellite images from Google Maps). 
%%Therefore, the rider has a smaller number of possible predictions for the driver's location, which would further reinforce the motivation behind our attack.
%This would remove the error due to misclassification (and thus reducing the size of $\mathcal{S}'_i$), since Satellite images allows the rider to exactly determine whether a point lies on road, irrespective of width of the nearby road.
%
%We would also like to note that many cities around the world do have a majority of 2 lane roads, and so our experiments give a fairly accurate idea of location recovery probabilities.
\end{compactlist}

\textit{Remark}.
We give a brief insight into the number of drivers inside a zone, which averages to 400. The zone demarcation proposed for New York by the authors of ORide was discussed briefly above. 
According to ride information for May 2019 in the NYC Uber-Dataset, a zone in Manhattan had at most 6,000 ride requests per day.  (We chose the month of May since it experienced the most ride-requests in the year 2019).
%The boroughs of Queens and Bronx combined, had around 12,000 ride requests per day. 
We make the same assumption that the authors of ORide did: the drop-off zone for a driver is her waiting zone for new ride requests. Moreover, as in ORide, we assume that the waiting time between a driver's drop-off event and her next pick-up event is at most 30 minutes. 
This would mean that during a ride-request event, the available drivers to answer this request are the ones who had a drop-off event inside that zone in the last 30 minutes since the ride-request. 
We considered the top 20 high-ride zones, and for each zone, grouped the ride requests for a day based on 30 minute intervals. 
Each 30 minute interval consisted of at most 400 drop-off events inside each zone. This would imply that when a ride request occurs at any time of the day, at most 400 drivers would be waiting in that zone to service this request. We stress that there are at most 400 drivers in all zone demarcations considered above, and as the zone size increases the density of drivers (the number of drivers available for ride request in 1 km\textsuperscript{2}) in that zone decreases.

%\vspace{-0.8cm}

\subsection{Impact and Consequences of our Attack}
\label{sec:impact_attack}

We have experimentally shown that our location-harvesting attack can identify the exact locations of a driver in about 45\% of the cases. Equivalently, this means that in a zone of around 400 available drivers, a ride request leaks the locations of around 180 drivers to the rider, which is a significant number. Although our attack doesn't reveal additional driver data such as user profiles, this leak of location information could still cause potential threats to drivers and ultimately affect the SP's reputation.
For instance, according to \cite{istanbul_uber}, it is claimed that non-SP taxi drivers try to identify locations of Uber vehicles and attack them. There are also reports of people using ride-hailing apps to locate and rob drivers registered to the SP \cite{thejournal}. Zhao et.~al.~\cite{Zhao2019GeolocatingDA} investigate several approaches through which information regarding drivers' locations can lead to statistical attacks and exploits. 
A potential competitor to ORide can use our attack and make queries to ORide as an honest-but-curious rider over a period of time.   It can then get to know the distribution/density of different drivers in the city without raising suspicions. This distribution could indicate regions where there is high demand for ride hailing services.
The competitor could focus on deploying their drivers and taxis in that region.

In general, ensuring privacy of the locations of drivers in the zone should be an important aspect of any privacy-preserving RHS. The authors of ORide claim that an adversary cannot obtain a snapshot of drivers' locations (say, a malicious rider who makes multiple fake ride requests with the goal of harvesting drivers' locations) \cite[\S8]{ORidePaper}, thus preserving their anonymity.
In contrast, our work refutes this claim made in ORide using just a single ride request by an honest-but-curious rider.
We think that this flaw in ORide is not merely an implementation error. The requirement of integer-encoded inputs is inherent to current SHE schemes, and this helps us obtain small number of lattice points on the circle. 


\textit{Remark. }
One of our motivations behind considering privacy of driver locations is to prevent physical attacks on the drivers in a zone. It can be argued that even if locations of these drivers are not revealed, a malicious rider can request a ride in an honest manner, and attack the chosen driver when she arrives at the pick-up location. 
While this is true, and in fact, at the end of any ride hailing service (whether it preserves privacy or not), the selected driver \textit{must} arrive at the rider’s pick-up location and so, this attack scenario is nearly impossible to thwart. However, in almost all apps (including ORide), the identity information of the rider (name, phone number etc.) is revealed to the driver selected for the ride (and vice-versa) which act as a 
deterrent for such attacks. 
The possibility of fake accounts can be eliminated by enforcing identity verification at the time of registration. This does not violate rider privacy since ORide assigns anonymous tokens to all entities during the ride request process. 
Using our attack from Section \ref{analysis}, a rider can get to know even the locations of \textit{non-selected} drivers in the zone, namely the other drivers who have no information about the identity of the rider. 
Finally, we remark that if the driver has moved from her last revealed location or does not have a logo/sticker on her car (advertising that she belongs to a particular RHS) then it would be hard for the rider to carry
out physical attacks.

%When the locations of drivers in the zone are revealed, there are two other situations in which physical attacks by the rider does not make sense. First, drivers could be moving, which means that by the time the rider arrives at the last known driver's location, she would not be there anymore. Second, a driver belonging to the SP may not have a logo/sticker on her car, advertising that she belongs to a particular RHS. This would make it harder for the rider to identify which car belongs to the driver. But, counter-arguments can still be made as follows --- normally, drivers wait at a particular location or will be moving within a small area while waiting for customers, meaning there is a high probability the driver will be present at or around the advertised location. In most of the cases, a driver belonging to a certain service provider will have a logo/sticker on the car, to help the rider identify the driver when she arrives at the pickup-point. We acknowledge that there are situations in which it is hard for the rider to physically attack a driver, given her last known location.


%We believe our attack should motivate future works in the security analysis of other privacy preserving solutions that use homomorphic encryption.
%\subsection{Euclidean distance as a metric for closeness}
%
%\label{euclidean_metric}
% 
%We motivate our newer solution proposed in Section \ref{solution}, by considering the accuracy of euclidean metric for ride-matching. 
%Clearly, the best metric for choosing the closest driver should consider the actual time it would take for the driver to reach the rider in the real world. 
%This metric should reflect road structures in the rider's location, traffic conditions, optimal routes (e.g., via freeways or inner city roads), etc. 
%These factors are not considered when we simply choose to measure closeness of a driver based on euclidean distance. 
%Hence, the best possible solution for the rider would be to use Google Maps Distance Matrix API to find out the actual time between her and a driver. 
%This API considers all the factors mentioned before and would be the perfect solution, giving 100\% accuracy when picking the closest driver.
%
%In ORide, the SP only sends to the rider, the encrypted euclidean distance information between the rider and each driver. 
%Hence, \emph{in the protocol of ORide}, the rider doesn't get the actual driver's coordinates, but only the euclidean distance to them. 
%With only this much information, the rider could not make use of Google Maps API to find out the actual time (since the rider doesn't have the drivers' coordinates).
%Hence, the next best thing that the rider could do, is use euclidean distance as the metric.
%
%We ran experiments to compare the accuracy of euclidean metric against the time metric. 
%Similar to our experiments in Section \ref{analysis}, we chose the same three cities --- Dallas, Los Angeles and London. In the explanation that follows, we shall use the same notations described in Section \ref{analysis}.
%For every city, each experiment first chose a random $\mathcal{G}_{3,3}$ inside $\mathcal{G}$. 
%Then, a random rider coordinate was chosen, and 50 random drivers were chosen inside $\mathcal{G}_{3,3}$. 
%Using Google Maps Distance Matrix API, the driver $d_{time}$ having the least actual time from the rider was found out. 
%Then, all rider and driver coordinates were converted into UTM, and the driver $d_{euclidean}$, having the least euclidean distance from the rider was found out.
%If $d_{euclidean}$ had the same actual time to the rider as $d_{time}$, then the accuracy of the euclidean metric was incremented (the euclidean metric correctly chose the driver having the least time).
%The above was repeated for $\mathcal{G}_{5,5}$ (with 75 drivers inside this zone) and $\mathcal{G}_{10,10}$ (with 100 drivers inside the zone).
%The collected results are shown in Table \ref{tab2}.
%
%\begin{table}
%\centering
%\begin{tabular}{| m{30pt} | m{35pt} | m{40pt} | m{50pt} | }
%\hline
%City & Zone Size (km\textsuperscript{2}) & Number of drivers in zone & Accuracy of euclidean metric\\ [3pt]
%\hline 
%\multirow{3}{1em}{Dallas} & 9 & 50 & 66.6\% \\
%& 25 & 75 & 53.3 \% \\
%& 100 & 100 & 60\% \\[3pt]
%\hline
%\multirow{3}{1em}{Los Angeles} & 9 & 50 & 66.6\% \\
%& 25 & 75 & 63.3\% \\
%& 100 & 100 & 53.3\% \\[3pt]
%\hline
%\multirow{3}{1em}{London} & 9 & 50& 40\% \\
%& 25 & 75 & 43.3\% \\
%& 100 & 100 & 56.6\% \\[3pt]
%\hline
%\end{tabular}
%\newline
%\caption{Averaged accuracy of the euclidean metric against time metric in choice of the closest driver}
%\label{tab2}
%\end{table}
%
%We have argued about our choices for sizes of these zones in Section \ref{analysis}. Now, we shall justify why we chose 50, 75 and 100 drivers in these zones. 
%If the SP decides to choose a smaller size for a zone, it would mean that this zone has more ride requests per km\textsuperscript{2} of area, to achieve the desired anonymity-set size (as in the case of a city like Los Angeles with higher population density). 
%Similarly, if the size of a chosen zone is larger, then it would mean that lesser ride requests occur per km\textsuperscript{2}, hence the need to chose a bigger zone to maintain the same anonymity-set size (as in the case of a relatively less dense city like Dallas). 
%
%If a zone has more ride-hailing activities, drivers would be motivated to wait for ride requests from this zone, and hence on average, more drivers would constantly be available for ride requests from a rider at each instant. 
%So, for a 3km x 3km zone (which should have more ride-hailing activities due to smaller size of the zone), the density of drivers available for ride request at an instant, per km\textsuperscript{2}, is high. 
%When we chose 50 drivers for a 3km x 3km zone, we concluded the average density of available drivers at an instant to be $50 / (3\times 3) = 5.55$ drivers per km\textsuperscript{2}. 
%Based on this number, when a rider requests for a ride, she would have to compare the euclidean distances of 50 drivers, and hence we chose 50 driver coordinates for $\mathcal{G}_{3,3}$.
%
%Similarly, a 5km x 5km zone would have relatively lesser driver density at an instant compared to a 3km x 3km zone (due to lesser ride-hailing activity). Indeed, with an average of 75 drivers at any instant inside $\mathcal{G}_{5,5}$, the density would be $75 / (5 \times 5) = 3$ drivers per km\textsuperscript{2}.
%
%A similar argument holds for 10km x 10km zones, with the average density being $100 / (10 \times 10) = 1$ driver per km\textsuperscript{2}. 
%So, the values 50, 75 and 100 were chosen to ensure a decreasing driver density with increasing zone size. Moreover, considering 50 drivers in a highly active 3km x 3km zone in a busy hour of the day is reasonable, and would help us understand how poorly the euclidean metric would perform in congested traffic situations and high count of ride requests.


%
%\begin{table*}
%\small
%\centering
%%\begin{tabular}{| m{30pt} | m{35pt} | m{60pt} | m{80pt} |}
%\begin{tabular}{| c | c | >{\centering\arraybackslash}m{90pt} | >{\centering\arraybackslash}m{90pt} |}
%%\begin{tabluar}{|c|c|c|c|}
%\hline
%%\vspace{3pt}
%City & Zone Size (km\textsuperscript{2}) & Average number of predicted locations for each driver & Percentage of experiments with exact driver prediction  \\
%%\vspace{3pt}
%\hline 
%\multirow{7}{*}{New York} & 1 & 1.46 & 67\% \\
%& 2 & 1.60 & 43\% \\
%& 4 & 1.46 & 67\% \\
%& 9 & 1.60 & 70\% \\
%& 25 & 1.90 & 57\% \\
%& 100 & 1.70 & 47\% \\
%& 400 & 2.16 & 54\% \\
%\hline
%\multirow{6}{*}{Dallas}  & 1 & 2.00 & 57\% \\
%& 4 & 1.43 & 73\% \\
%& 9 & 1.53 & 67\% \\
%& 25 & 1.70 & 60\% \\
%& 100 & 1.76 & 53\%  \\
%& 900 & 1.70 & 50\% \\[3pt]
%\hline
%\multirow{6}{*}{Los Angeles} & 1 & 1.56 & 63\% \\
%& 4 & 1.80 & 43\% \\
%& 9 & 1.80 & 53\% \\
%& 25 & 2.23 & 50\% \\
%& 100 & 1.96 & 60\% \\
%& 900 &  1.83 & 50\% \\[3pt]
%\hline
%\multirow{6}{*}{London} & 1 & 1.23 & 80\% \\
%& 4 & 1.40 & 70\% \\
%& 9 & 1.63 & 63\% \\
%& 25 & 1.50 & 70\% \\
%& 100 & 1.73 & 53\% \\
%& 900 & 1.66 & 60\% \\[3pt]
%\hline
%\end{tabular}
%\newline
%\caption{Results of the rider's prediction analysis based on Algorithm \ref{algo:cryptanalysis}, averaged over 30 experiments for each zone size inside each city}
%\label{tab1}
%\end{table*}



==> sac arXiv version/fix.tex <==
\section{Mitigation of our Attack}
\label{sec:fix}

We propose a solution where the driver can thwart our attack by anonymizing her location. Each driver could choose a random coordinate within a circle of fixed radius around herself, encrypt and send these random coordinates to the SP instead of her original coordinates. We show that this modification to ORide provides sufficient anonymity while preserving ride matching accuracy, and is therefore a reasonable solution to mitigate our attack.   The idea of adding noise to geographical data to preserve privacy has been addressed in
several works in the literature. In Section \ref{sec:relatedwork}, we discuss some of these techniques and their relevance to our setting.
We analyze the effect of this technique on driver anonymity and provide concrete values for ride matching accuracy through experiments using Google Maps API.

\textit{Remark.} In Appendix \ref{further_attacks}, we discuss other ideas that may intuitively seem to thwart our attack. However, we show that those modifications are vulnerable to our attack from Section \ref{sec:cryptanalysis} and hence do not preserve driver anonymity.

\subsection{Anonymizing Driver Locations}
\label{sec:fix_idea}
%If we recall the protocol of ORide, each driver $D_i$ encrypted her current geographical coordinate (which by our assumption was on road, refer to Section \ref{analysis}) and sent it to the SP. During the rider's attack proposed in Section \ref{analysis}, she obtains all lattice points corresponding to the Euclidean distance between herself and $D_i$. 
%Now, if a lattice point did not lie on road (which the rider verifies using Google Maps API), she discards this lattice point. This is because since each driver is assumed to be on road, any lattice point that does not lie on road can never be a possible location for a driver.

By anonymizing her location, each driver may try to preserve the privacy of her location with respect to a rider.
Let each driver $D_i$ (at coordinates $L_i$) choose a circle of radius $R$ centered at her location (where $R$ is publicly known), and pick a random UTM  coordinates $L_i'$ inside this circle. The driver encrypts $L_i'$  (instead of $L_i$ as suggested by ORide) and sends it to SP. We refer to $L_i'$ as the anonymized driver coordinates.

As per the original attack in Section \ref{sec:cryptanalysis}, the rider obtains a Euclidean distance $N_i$ and enumerates all lattice points that correspond to this distance. Due to the changes described above, these lattice points need not correspond to possible driver coordinates. They instead represent possible \textit{anonymized} driver coordinates. 
The rider would have next proceeded to filter each lattice point based on whether it is on road or not. But a lattice point which represents an anonymized driver location may not lie a point on road, although the original driver did. Filtering in this way would lead to erroneous conclusions by the rider, and she may throw out a lattice point that actually corresponds to the driver location. 

Observe that within distance $R$ of anonymized driver coordinates, there will always lie a road (since the original driver was on road). We modify the rider's attack accordingly to cope with this fix. Suppose there was a lattice point discovered by the rider. Within a circle of radius $R$ centered at this point, if there were no roads at all (for instance a lattice point that was in the middle of a park) the rider can then conclude that this point is not the driver's anonymized coordinates. So, the best option that a rider has (to improve her attack against this obfuscation technique) is to filter each lattice point based on whether there is a road within distance $R$ of that point. 
As we see in Section \ref{sec:effect-on-anonymity}, the possibility that a lattice point is filtered out in a dense city is low if we choose an appropriate value of $R$. This prevents a rider from eliminating many lattice points thus improving driver anonymity. Moreover, this technique preserves accuracy when compared to ORide as we show next. 


%\subsection{Effect on Anonymity and Ride-Matching}
%\label{sec:fix_accuracy}

%We ran experiments in the city of New York and Los Angeles and observed the effect of this obfuscation technique on driver anonymity and ride-matching. 

%We performed experiments implementing this obfuscation technique at drivers' end and running the modified attack at the rider's end. We considered the cities of New York and Los Angeles with zone sizes of 1 km\textsuperscript{2}, 2 km\textsuperscript{2} and 4 km\textsuperscript{2} (as described in Section \ref{practical_implementation}). Our experiments below to check drivers' anonymity and ride-matching accuracy averaged the results over these zone sizes  and considered 400 drivers in each zone.
  
\subsection{Anonymity of Drivers with respect to Rider}
\label{sec:effect-on-anonymity}

The value of $R$ is public and should be decided by the SP, who can in fact implement the end-user application in such a way that the driver's device locally computes $R$ based on the current location of the driver. If the driver's local device senses that she is in a densely populated city (and thus there are many roads within close proximity of an arbitrary point in that region of the city), a smaller $R$ can be chosen. On the other hand, if the device understands that the driver is in a location where there are very few roads within distance $R$ from an arbitrary point in that region, a larger $R$ is chosen (for instance, in a sparsely populated city with low road density). This choice of $R$ based on the concentration of roads around the driver is motivated by the modification to rider's attack discussed at the end of  Section \ref{sec:fix_idea} (the rider's attack now tries to filter lattice points based on the availability of roads within distance $R$ from each lattice point solution).
We consider the number of (anonymized) driver locations predicted by a rider as a measure of anonymity for that driver. This depends on the number of lattice solutions for the Euclidean distance between (anonymized) driver location and rider. Along with this, it also depends on the number of solutions that the rider can further filter based on availability of roads within distance $R$ from each solution. We expect anonymity to increase with $R$ due to higher probability of finding a road within distance $R$ of any location.

Similar to the setup in Section \ref{practical_implementation}, in the following discussion we average results over 25 experiments where each experiment chooses a random zone of size 4 km\textsuperscript{2} in the mentioned city (along with random coordinates for a rider and driver) and runs the modified rider's attack for filtering coordinates.
For a small value of $R$ such as 10 m, any coordinate within distance $R$ of some point is practically the same location.
We experimentally observed that the average anonymity for a driver in Los Angeles was around 3, which is close to what we observe in the original attack (see Table \ref{tab1}). Hence small values of $R$ should not be chosen since they offer low anonymity. 
In a densely populated city such as Los Angeles, most locations within the city are expected to have roads within reasonable distance. For $R=$~50~m  we observed that the area surrounding \textit{most} lattice points in Los Angeles had at least one road within 50~m. From a rider's perspective, this would mean that most lattice solutions obtained by her are possible choices for the anonymized driver coordinates. Experiments showed that the average number of filtered lattice points when $R=50$~m was 14 (meaning the rider has 14 possible \textit{anonymized} locations of a driver). This provides sufficient anonymity to a driver in practice, since the probability of correctly predicting a driver's anonymized coordinate is only $1/14$.   This is certainly an improvement compared to $1/1.8$ for ORide (Table \ref{tab1}).
Considering Dallas, a city with relatively sparse road density, we observed that a significant number of locations did not have roads within 50~m, and this allowed the rider to filter out many possible lattice solutions. Our experiments suggest that choosing $R=150$ m prevents the rider from doing so and offers sufficient anonymity, which averaged around 16.

\textit{Remark.} 
As seen above, the rider ends up with around 15 equally probable solutions for the driver's obfuscated
location.  This means that even if the rider applies clustering algorithms over multiple queries to eliminate noise and tries to find the actual driver’s location, there will still be many equally probable locations for the driver ($>10$) thus providing high anonymity.


\subsection{Accuracy of Ride-matching}
When a driver chooses random coordinates within distance $R$ instead of her own location, the Euclidean distance is now computed between the rider's location and the \textit{anonymized} driver location. %Consequently, this leads to decreased efficiency in ride-matching when compared to the Euclidean metric between rider and driver location as in ORide. 
%The decrease is more amplified since there are around 400 drivers in a small zone. (The sizes of zones is relatively small in dense cities, refer to Section \ref{practical_implementation}). 
%Our experiments compared the number of executions where the closest driver chosen by the Euclidean metric was same in both cases (i.e., in the non-anonymized approach used by ORide  against the anonymized approach used here).

%We evaluate the ride matching accuracy of a metric relative to the time-based metric (Google Maps API was used to determine the time-wise closest driver). 
%Concretely, we measure the accuracy of a metric as the percentage of experiments in which the optimal driver chosen by this metric is within 1 minute away from the time-wise closest driver (A window of 1 minute is reasonable and provides sufficient error margin for the chosen metric in practice).
Among all drivers in the zone, suppose an optimal driver is chosen according to some metric $M$. For example, if $M$ represents Euclidean distance, the optimal driver is the one with least Euclidean distance from her location to the rider in the case of ORide, and the one with least Euclidean distance from her anonymized location to the rider in the case of our modified solution. Let $t_M$ be the time taken for this optimal driver to reach rider. Let $t_T$ be the minimum time taken among all drivers in the zone to reach rider (corresponding to the time-wise closest driver).
We evaluate the accuracy of metric $M$ as the percentage of experiments in which $|t_M-t_T|$ is less than or equal to 1 minute (in practice it is okay for the rider to wait another extra minute compared to the time-wise closest driver). Google Maps API was used to determine the time taken for a driver to reach the rider.

We chose zones of %sizes 4 km\textsuperscript{2}, 25 km\textsuperscript{2} and 100 km\textsuperscript{2}
varying sizes in Los Angeles and Dallas. In each experiment a random rider and 400 drivers were chosen in each zone.
We compared the accuracy of Euclidean metric for $R$ = 50~m and $R$ = 150~m in both scenarios -- when used in the context of ORide (computed between the rider and driver's actual location) and when used in the fix to our attack (computed between the rider and driver's anonymized location). As discussed previously, we chose $R=50$~m for Los Angeles and $R=150$~m for Dallas, respectively, to ensure sufficient anonymity. Moreover, the sizes of zones are chosen to be smaller in Los Angeles (refer Section \ref{practical_implementation}) and larger in Dallas. 
The inferred accuracies were averaged over 25 experiments (refer Table \ref{table:anony-accuracy}). We see that our solution indeed provides sufficient driver anonymity with respect to rider while preserving accuracy of ride matching compared to ORide. 

Choosing large $R$ to achieve greater anonymity in a small zone (where driver density is high) leads to loss of accuracy. This seems intuitively correct, since having a large anonymity radius in a small zone with high driver density greatly changes the ordering of drivers based on Euclidean distances. To concretely verify this, we used a similar setup described above and observed that with $R$ = 150~m and a 4 km\textsuperscript{2} zone size in Los Angeles the accuracy of ORide was around 84\% whereas that of the modified solution was only 70\%. So, $R$ should increase with zone size both to preserve accuracy and driver anonymity (prevent filtering of lattice solutions based on availability of roads).

\begin{table}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Comparison of accuracy of selecting best driver in ORide vs. our solution (with anonymized driver locations), averaged over 25 experiments.}
\label{table:anony-accuracy}
\centering
\begin{tabular}{l|c|c|c|c}
%\hline
City & Zone & Radius & ORide & Our\\
      & Size (km\textsuperscript{2}) & $R$  (m)  &  & solution\\
\hline
\multirow{3}{5em}{Los~Angeles} & 4 & 50 & 84\% & 80\% \\
& 25 & 50 & 92\% & 90\%\\
%& 100 & 33\% & 18\\
\hline
Dallas & 100 & 150 & 83\% & 83\%\\
%& 50 & 25\% & 12\\
%& 100 & 12\% & 14\\
%\hline
\end{tabular}
\end{table}

%In Los Angeles, for the values of $R$ being 10~m, 50~m and 100~m, the average ride-matching accuracy as per the obfuscation technique was on average 73\%, 46\% and 33\%, respectively. The accuracy in New York was on average 63\%, 25\% and 12\%, respectively.  
%We see that although this technique provides sufficient driver anonymity (for values of $R$ other than 10~m) and overcomes the rider's attack proposed in Section \ref{analysis}, it leads to a significant decrease in accuracy compared to ORide. We believe that this is not a practical solution to the problem of driver-location privacy (with respect to riders) that exists in ORide.


==> sac arXiv version/further_attacks.tex <==
\appendix
\vspace{-0.15in}
\section{Appendix : Further Attacks}
%\section{Further Attacks}
%\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection}}
\label{further_attacks}
We look at potential ways in which our attack can be thwarted and analyze their efficacy.  In the first scenario, in order to obfuscate driver locations, the SP homomorphically adds  noise to driver distances before sending them to the rider. %This is done, for instance, by computing a random monotonically increasing polynomial function of the distances that preserves the ordering of the distances but hides the actual values to make our original attack possibly ineffective.
 For this case, we show that a rider can still break anonymity by recovering the original distances between the rider and the drivers.  
 %In the second scenario, the driver herself adds random noise to her location by choosing a random coordinate within a fixed distance from her before sending it to the SP.   We find that in such cases while privacy is maintained for sufficiently large noise, there is considerable loss in accuracy of rider selecting the closest driver when compared to the Euclidean metric. 
 In the second scenario, the SP uses $p$-norm metric instead of the Euclidean distance and we show that our attack also extends to this case.
Note that increasing zone sizes is not a countermeasure to our attack. As discussed in Section \ref{practical_implementation}, zone sizes should be small enough (less than 1000 km\textsuperscript{2} in practice) to ensure efficient ride-matching times and lower bandwidth costs.
 
%\textit{Remark}.
%The following two techniques, although straightforward to think of, fail to provide an effective countermeasure to our attack. We believe that preserving driver locations' privacy w.r.t.~riders in ORide remains an interesting open problem. Any other countermeasure seems to be non-trivial to come up with and is beyond the scope of the current work.

\vspace{-0.1in}
\subsection{Homomorphic Noise Addition by SP}

In order to thwart our attack, the SP could try to obfuscate driver locations by
%homomorphically add to each (encrypted squared) Euclidean distance a constant noise $\delta$, where the noise can be a randomly selected integer that is possibly large. A more general approach is for the SP to 
transforming the (encrypted squared) Euclidean distances using a random monotonic polynomial $F$ with integer coefficients and of a small degree, as suggested by Kesarwani \etal \cite{KesarwaniKNPSMM18}. 
Integer coefficients are needed for ease of representation in homomorphic computations, monotonicity is needed to maintain the sorting order of the distance inputs (so that the rider obtains the correct order upon decryption), and low polynomial degree is required for efficient homomorphic evaluation.
%This would maintain the original ordering that was present among the (squared) Euclidean distances, since a monotonic polynomial is used. 
Let $N_i$ be the Euclidean distance between the rider and a driver $D_i$ in her zone.
The rider would get to know from the SP, for each driver $D_i$ in her zone, the values $F(N_i)$ for some random monotonic integer polynomial $F$ of low degree. Note that $F$ is unknown to the rider, but the degree $d$, range of coefficients of the polynomial $[1,2^\alpha -1]$ and range of $N_i$ ($[0,2^\beta -1]$) are publicly known. We claim that the rider can obtain the actual distance $N_i$.

\cite{MurthyV19} provides a method of recovering a monotonic integer polynomial of low degree and bounded input range when only sufficiently many outputs evaluated at integer points are provided.  We used the publicly available SageMath \cite{knnpolycode} code from the authors of \cite{MurthyV19} with parameters similar to that described in \cite{KesarwaniKNPSMM18}, namely $d = 9$, $\alpha = 32$ and $\beta = 28$. 
% TIFS We pick a degree-9 monotonic polynomial with uniform random coefficients in the range $[1,2^\alpha -1]$ where $\alpha=32$, and integer inputs are in the range $[0,2^\beta -1]$ where $\beta=28$.
%We note that the polynomial must be of low degree ($\le 9$) for efficiency of homomorphic operations and $\beta=28$ is sufficient to represent values in the input domain (for smaller zone sizes, 28 bits are enough to represent squared Euclidean distances). 
%The choice  $\alpha=32$ provides a seemingly sufficiently large space of monotonic polynomials to choose from \cite{KesarwaniKNPSMM18}.
Next one obtains outputs $F(N_i)$ by evaluating this polynomial on the distances $N_i$.  These two steps are the same as what the SP would do (homomorphically) once it receives inputs from the rider and all drivers in a particular zone.  The $F(N_i)$ values, $d$, $\alpha$ and $\beta$ are the only values given to the SageMath code in the experiments to recover (squared) Euclidean distances to drivers for various zone sizes.  We correlated back the results of the recovery with the input distances and verified that in all cases the recovered distances matched correctly, which means that the rider can proceed with the attack mentioned in Section \ref{sec:cryptanalysis} after recovering $N_i$ values.   
%The result of recovery of the distances in various zone sizes and the time to recover is given in Table \ref{tab:ni_recovery}.
%, following which the polynomial outputs are sent to the rider for decryption, sorting and driver selection.

%In our scenario, the polynomial inputs (i.e., the squared Euclidean distances) come from a range that is feasible to enumerate even for a very large zone size.

%For completeness, we give a brief description of the method used in \cite{MurthyV19} for integer polynomial and input recoveries.   They make use of the fact that all the input values are non-negative integers which will reduce the search space drastically compared to the real numbers.  Their main idea is to extract differences in the inputs since the difference between two input values is an integer divisor of their respective polynomial outputs.   For this they find all divisors (and hence differences) within a bound since it is known that the input values themselves are bounded.   They then compute differences between divisors of multiple pairs and form a consistent set with just the right number of differences needed to reconstruct the polynomial (degree of which is known publicly).   Finally they use Lagrange Interpolation to recover the degree-d polynomial with the $y$-values coming from $d+1$ polynomial outputs and the $x$-values are formed such that the smallest (corresponding to the smallest of the $y$-values) $x$-value is an unknown parameter, say $x_0$, and the other $d$ values come from the consistency set.  Next they iterate over integer values of $x_0$, starting from $x_0 = 0$, and in each step recreate the polynomial and examine the coefficients.  Since the bounds on the coefficients is known, unsuitable polynomials are discarded until a polynomial that satisfies all conditions is obtained, and the algorithm stops with  the first such polynomial, and the value of $x_0$ and the differences therein are output.  They claim in the paper that with a high probability they can recover the polynomial that satisfies the /given set of outputs and their corresponding input values. 

% TIFS In order to exactly mimic the rider scenario, the inputs given to the SageMath code in our experiments only include the values $F(N_i)$, degree of the polynomial used, range of the polynomial coefficients and range of $N_i$.  

%We ran experiments to recover (squared) Euclidean distances to drivers for zones of various sizes.  We correlated back the results of the recovery with the input distances, and verified that in all the cases the recovered distances matched the input distances.  The result of recovery of the distances in various zone sizes and the time to recover is given in Table \ref{tab:ni_recovery}.  Based on these results we see that the rider can indeed very likely recover the values $N_i$ and can proceed with our attack mentioned in Section \ref{sec:cryptanalysis}.

%\begin{table}[!t]
%\renewcommand{\arraystretch}{1.3}
%\caption{Time taken to recover $N_i$ and the monotonic polynomial for different zone sizes}
%\label{tab:ni_recovery}
%\centering
%\begin{tabular}{c|c|c|c|c|c|c}
%%\hline
%Zone size (km\textsuperscript{2}) & 1 & 4 & 9 & 25 & 100 & 900\\
%\hline
%Time (seconds)  & 38 & 54 & 60 & 274 & 934 & 7469\\
%
%%\begin{tabular}{|c|c|}
%%\hline
%%Zone size (km\textsuperscript{2}) & Time (seconds)  \\
%%\hline
%%1 & 38 \\
%%4 & 54 \\
%%9 & 60 \\
%%25 & 274 \\
%%100 & 934 \\
%%900 & 7469 \\
%%\hline
%\end{tabular}
%\end{table}
%
%\end{enumerate}

\vspace{-0.1in}
\subsection{$p$-norm Metric by SP}
\label{sec:p-norm}
In order to mitigate our attack in Section \ref{sec:cryptanalysis}, the SP may try to homomorphically compute the $p$-norm (instead of Euclidean distance) of ciphertexts and send it to rider. Let $(x_R, y_R), (x_{D_i},y_{D_i})$ denote coordinates of a rider and driver $D_i$, respectively. The rider would thus obtain $N_i = |x_R-x_{D_i}|^p+|y_R-y_{D_i}|^p$ for each driver $D_i$ in her zone (the value of $p$ should not be too large to allow efficient homomorphic computations by SP).

Note that if $p$ is odd, $(x_R-x_{D_i})^p+(y_R-y_{D_i})^p$ could represent a negative value. Since ORide uses \textit{ciphertext packing} and non-Boolean circuit representation with the underlying SHE library \cite{ORidePaper}, it is very inefficient to compute the absolute value homomorphically. 
% When such negative values occur, $c_{dist}$ would correspond to a negative value that is taken modulo some integer. In this case, the value of $N_i$ would not correspond to $(x_R-x_{D_i})^p+(y_r-y_{D_i})^p$, and the ordering of closest drivers would be different from what is interpreted through $N_i$. So, to allow the rider to accurately choose the closest driver (by choosing the least $N_i$ value), 
Hence, the SP would have to use only even values for $p$.
Let $p=2q$. In the rider's attack, she has to now enumerate all lattice points satisfying the equation $x^p+y^p=N_i$. Observe that if $(x,y)$ is a solution to this equation, then the lattice point $(x^q, y^q)$ is a solution to $x^2+y^2=N_i$. This implies that the solution set comprising of lattice points satisfying $x^p+y^p=N_i$ is smaller than the solution set of lattice points satisfying $x^2+y^2=N_i$. Based on our experiments on various zones and cities, we have estimated the number of lattice points satisfying $x^2+y^2=N_i$ to be around 20 (refer to Section \ref{practical_implementation}). This means that on average, the lattice points satisfying $x^p+y^p=N_i$ cannot be greater than 20 in number. The rider (similar to the rest of the attack) can then check whether each lattice point lies in the zone and on road, to reduce the number of possible predicted driver locations. In this way, our attack also applies when the SP uses $p$-norm instead of Euclidean distance. 

%\textit{Remark}.
%The above three techniques, although straightforward to think of, fail to provide an effective countermeasure to our attack in Section \ref{sec:cryptanalysis}. We believe that preserving driver location privacy w.r.t.~riders in ORide remains an interesting open problem. Any other countermeasure is non-trivial to come up with and is beyond the scope of the current work.



==> sac arXiv version/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Ride Hailing Services such as Uber, Lyft are becoming popular world-wide year over year. According to Pew Research \cite{pew:rhs_research}, the number of Americans who have used RHS has more than doubled since 2015.   In order to provide the service, RHS Service Providers (SP) collect upfront information about individuals desiring to use their services, which include riders and drivers who are part of the network.  In addition, details of rides offered and accepted are also collected as part of their billing and statistics gathering.  
%While these seem natural to the service provider, it 
This raises a number of privacy concerns among the individual users.   
%Information regarding the drivers and riders are collected by the provider at the time of subscription.  And every ride taken by a rider is also recorded for the purposes of billing and statistics.  
Though the SP would, in general, keep the information secure given the need to keep its reputation high, there is nothing to prevent breach of privacy if either the provider turns malicious or if someone with access to information internal to the provider wants to mine the information for personal gain  \cite{norton_databreach}.

A ride hailing service consists of three parties, namely, the SP, a rider who has subscribed for services of the SP and a set of drivers involved in ride selection.  The SP is modeled as an honest-but-curious adversary.  We consider the threat model where the rider attempts to mount a location-harvesting attack on participating drivers.  While there are a number of solutions proposed in the last few years that preserve privacy of riders and drivers with respect to the SP, there are only a few works that look at privacy issues of drivers with respect to riders.  The work {\em Geo-locating Drivers} \cite{Zhao2019GeolocatingDA} does an analysis of features and web APIs of non-privacy preserving RHS apps which can be used to extract privacy sensitive driver data.    {\em PrivateRide} by Pham \etal \cite{Pham2017PrivateRideAP} describes how riders or other malicious outsiders posing as riders can harvest personal information of drivers for purposes of stalking, blackmailing or other malicious activities.  Apart from user-profiling, there are several instances where leakage of information regarding driver locations can lead to serious threats (refer Section \ref{sec:impact_attack}). % The article \cite{thejournal} reports of how a gang  makes use of ride-hailing apps to harvest driver locations for robbery.  Another article \cite{istanbul_uber}, claims that some regular (non-SP) taxi drivers, pretending to be customers, located Uber vehicles to attack them.  These incidents provide a motivation to consider driver-threat models that leak locations of drivers to riders.

One of the early privacy-preserving ride hailing services is {\em ORide} \cite{ORidePaper}.  While the primary focus of this proposal was to provide an oblivious ride-matching solution to riders while preserving the privacy of riders and drivers from the SP, it also considers
location-harvesting attacks against drivers by a malicious set of riders who create and cancel fake ride requests simultaneously from  multiple locations.   
ORide ensures the anonymity of the drivers and riders with respect to SP primarily through the use of a Somewhat Homomorphic Encryption (SHE) scheme.  
%In addition to using anonymous payment modes, it provides accountability as well as a number of user convenience features.  
There are more recent works that also propose privacy-preserving RHS, and an overview of the works related to RHS is given in Section \ref{sec:relatedwork}.  
%In terms of completeness of the solution along with ease of use and deployment with current non-privacy-preserving RHS systems, we believe that ORide is still relevant and useful as a privacy-preserving RHS.

In ORide, the SP collects SHE encrypted coordinates of the 
drivers in the zone of the rider, homomorphically computes the Euclidean distances between the rider and drivers, 
and then sends these encrypted values to the rider. The rider then decrypts the encrypted distances, chooses the 
nearest driver and proceeds with ride establishment (the ORide protocol is recalled in Section \ref{oride_intro}).
This clearly leaks the distances of even those drivers who were {\em not} selected to offer the ride. But given that there are many possibilities for the coordinates of the driver, even if only their distance is known, one would expect that in practice the exact driver location is anonymous.
However, we show that while the protocol hides personal information of the drivers it offers only limited anonymity for the drivers' locations w.r.t.~a rider who requests a ride. 

\subsection{Our Contribution}
In this work, we show a location-harvesting attack on the drivers in the ORide protocol.
Along with the privacy for riders and drivers with respect to the SP, ORide also claims that its design  offers location privacy for drivers with respect to riders by preventing location-harvesting attacks. 
This is done using deposit tokens and permutation of driver indices for each ride request, which prevents a malicious rider from making fake ride requests and triangulating locations of all drivers in the zone \cite[\S8]{ORidePaper}. 
We show in Section \ref{analysis} that even an honest-but-curious rider, with only one ride request and response, can recover the exact coordinates of about half the number of drivers who respond to her ride request. Such an attack is not easy for the  SP to detect unlike attacks that involve simultaneous ride requests and cancellations.  We remark here that except driver location information, no personal driver information is revealed in our attack.
Nonetheless, in Section \ref{sec:impact_attack} we discuss practical scenarios where revealing only
the drivers locations (without their identities) can be harmful.


%Some works that follow ORide (\cite{pRideLuo}, \cite{lpRideYu}) only send information about the optimal driver to the rider, and not that of other drivers in the region (unlike ORide which sends Euclidean distance of all drivers in the zone). An important distinction is that our work targets anonymity of all other drivers in the region with respect to rider, since the location of the optimal driver is anyway revealed to rider once ride establishment is completed. Therefore it is not meaningful to extend our attack to works that only send information about optimal driver and our attack is relevant whenever location of all drivers are sent to the rider. 
%%To stress the impact of our attack, the importance of maintaining location privacy of drivers with respect to a rider (and not just the SP) has been discussed in Section \ref{sec:introduction}. 

Our attack is motivated by the classical 
\textit{Gauss' circle problem} \cite[Ch. 9]{takloo2018pythagorean}. ORide uses a map-projection system such as UTM \cite{UTMGrid} to work
with planar integer coordinates. Recovering the integer coordinates $(X_d, Y_d)$ of the driver 
by the rider reduces to solving  $(X_r-X_d)^2 + (Y_r-Y_d)^2 = N$, where $X_r,Y_r,N$ are non-negative integers 
that are known to the rider. Relabelling this equation as
$x^2 + y^2 = N$ results in a variant of the Gauss' circle problem. Since $N$ is sufficiently small, it is feasible to enumerate all the lattice points (i.e., 
points with integer coordinates) on the circle of radius $\sqrt{N}$. In our case, since $N$ always 
corresponds to the case where a solution is known to exist, we experimentally observe that 
the number of solutions to be about $20$ on average (over our choice of zones in Table \ref{tab1}). Then we 
use the following ideas to further eliminate the potential solutions: (i) the driver coordinates must be in the same zone
as that of the rider, (ii) the driver is typically expected to be at a motorable location such as road 
though the rider can book the ride from anywhere. This allows us to eliminate most of the 
possibilities (see Algorithm \ref{algo:cryptanalysis} in Section \ref{sec:cryptanalysis}) and reduce the number of solutions from 20 to about 2 on  average. 
In Section \ref{practical_implementation}, we validate our attack by running experiments over 
zones of different sizes for four arbitrarily chosen big cities, and show that a rider can determine the 
\textit{exact} locations of 45\% of the responding drivers (see Table \ref{tab1}). Our attacks take an
average only 2 seconds per driver on a commodity laptop.
We stress that we are not only using the geographical information to eliminate locations, but also the fact that all coordinates are encoded as integers and hence there are only a handful of locations to enumerate on the circle in the first place. 
Our attack exploits an inherent property of SHE schemes -- namely the requirement of integer-like encoded inputs for \textit{exact} arithmetic \cite{SAC:CSVW16}. We also believe that the abstraction of our attack as enumerating lattice points on a circle (and also our extension to other distance metrics in Appendix \ref{further_attacks}) is generic and will motivate similar exploits in other privacy preserving solutions that use SHE.
%Section \ref{sec:impact_attack} briefly describes the practical consequences and impact of revealing driver locations to the rider.

%Our work demonstrates that achieving location privacy of drivers w.r.t. riders (while still maintaining the desired privacy guarantees and ride-matching accuracy) in ORide is an open problem.

In Section \ref{sec:fix}, we propose a modification to the ORide protocol which serves as a solution to overcome our attack. Here the driver obfuscates her location by choosing random coordinates within a certain distance $R$ from her original location. Now the rider receives Euclidean distances that are homomorphically computed between her and the driver's anonymized location. Accordingly we modify the rider's attack from Section \ref{sec:cryptanalysis} to account for the fact that these anonymized coordinates (which are represented by different lattice solutions) may not lie on road. However the anonymized coordinates will definitely have a road within proximity $R$, since the driver was originally on road. Through experiments we analyze this new attack on the proposed modification and evaluate its effect on driver anonymity and accuracy (refer Table \ref{table:anony-accuracy}).
The optimal driver chosen in this case (based on least Euclidean distance between the rider and anonymized drivers'  locations) is sufficiently close to the time-wise closest driver (who takes the least time to arrive at rider's location). Our solution is therefore viable in practice and is successful in preserving driver anonymity.

%We think that this flaw in the original ORide protocol is \textit{not} merely an implementation error but one that is inherent to current SHE schemes. %Our objective is to motivate future works in the security analysis of other privacy preserving solutions that use homomorphic encryption.
%Although our attack turned out to be rather easy to fix, %it showed an inherent limitation in ORide that was not considered by the authors of that work. Also, 
%our modified solution is not ideal in the sense that we lose some accuracy (though it seems quite acceptable in practice). We believe that any solution that fixes this flaw in ORide without drop in accuracy is deeply linked with the open problem of efficient sorting on encrypted data.

In Appendix \ref{further_attacks}, we investigate possible alternate modifications to ORide in an attempt to mitigate our attack. However we show that these non-trivial techniques are eventually vulnerable to the same attack. % In Appendix \ref{appendix_b}, we give the full algorithm for our attack.

In Section \ref{sec:relatedwork}, we discuss related works on privacy-preserving RHS and also briefly discuss the applicability of our attacks to these works.   We also discuss other techniques
that are available in the literature for location obfuscation.

%We particularly focus on two modifications that result in the same driver being selected to offer ride as that of the original ORide protocol.   
%and look at tradeoffs that are involved therein.  
%or lead to a significant loss in ride-matching accuracy, and hence are not feasible in practice.
%In the first scenario, the SP can (homomorphically) perturb the driver Euclidean distances while still maintaining ordering of the distances to prevent riders from exploiting the actual Euclidean distances.  But it is possible to recover the actual values and hence mount our original attack by making use of a recent technique from \cite{MurthyV19} to recover integer inputs given the integer polynomial outputs.  
%In the second scenario, the drivers themselves obfuscate their locations by adding a random noise.  In this case we show that, while the driver enjoys higher anonymity, the accuracy of the nearest driver selection decreases considerably even compared with the Euclidean metric. 
%In the second scenario, the SP could use a $p$-norm metric (instead of the Euclidean distance) to match closest drivers. However, our attack naturally carries over to this case and such an attempt does not thwart our attack. 

%The design of ORide has inspired many recent works, many of which have been referenced in Section \ref{sec:relatedwork}.  Our attack on ORide can potentially motivate a critical look into privacy of more recent works. 

%Section \ref{sec:relatedwork} presents related works in the area of privacy preserving RHS. We conclude our paper and present ideas for future work in Section \ref{sec:conclusion}.


==> sac arXiv version/relatedwork.tex <==
\section{Related Works}
\label{sec:relatedwork}

%We primarily consider here references related to privacy preserving ride-hailing services.  
%We also consider some ride-sharing services that specifically deal with driver privacy.  
%We look at techniques that aim to anonymize private data.

Among providers of RHS namely Lyft, DiDi, OLA, taxify and others, Uber is one of the popular ride service providers.  An in-depth analysis of the practices followed by Uber and the impact of price-surging on passengers and drivers are done by Chen \etal \cite{Chen2015PeekingBT}. {\em The Guardian} \cite{guardianReport} reports how anonymized details of New York city taxi drivers can be used to easily convert the data to its original format to  obtain personal information.
Different threat models are widely considered in the literature, namely, a malicious driver targeting riders, and an honest-but-curious SP harvesting information about riders and drivers with the intention of selling it to other entities for advertising purposes, or with potentially malicious intentions to target high profile individuals.  Privacy of the driver is given much less attention; so much so that in a few papers the actual driver locations are revealed to the SP as well as the rider \cite{khazbak}  and \cite{raza_bride}.   As motivated in Section \ref{sec:introduction} there can be instances where a malicious rider can target drivers of a specific SP.    For example, a competitor SP can masquerade as rider to collect driver profile information or statistics to target the drivers belonging to the specific SP.  
{\em Geo-locating Drivers} by Zhao \etal\cite{Zhao2019GeolocatingDA} does a study of leakage of sensitive data, in particular, it evaluates the threat to driver information.  They show it is possible to harvest driver data by a malicious outsider SP by analyzing APIs in non-privacy preserving apps provided to drivers by Uber, Lyft and other popularly deployed SPs. \linebreak
% which might reveal location and driver details.  Attackers can also harvest significant driver information by requesting and cancelling rides continuously.  One of the countermeasures that an SP can take to prevent this is to rate limit such actions.   But it is not always be successful as the adversary can create multiple rider accounts to beat the system.  Another action by the SP is to penalize such cancellations, but it is not always enough especially if it is done by a malicious organization or competitor SP.
%The works \cite{Pham2017PrivateRideAP,ORidePaper} hide details of the ride in order to address the privacy concerns of the rider.  
\indent {\em  PrivateRide} by Pham \etal \cite{Pham2017PrivateRideAP} is one of the first papers to address privacy in RHS.  The location of the riders are kept hidden by means of a cloaked region, and location privacy is preserved by using cryptographically secure constructs.  Details of rider and selected driver are mutually exchanged
only after the ride request is fulfilled and when they both are in close proximity, to prevent a malicious outsider
trying to harvest driver information.
A recent work by Khazbak \etal \cite{khazbak} improves upon the solution of {\em PrivateRide} by providing obfuscation techniques (spatial and temporal cloaking), of rider locations, to achieve better results in terms of selecting the closest driver, at the cost of slightly more computational overhead.   However, the drivers' locations are revealed to the rider.  \\
%They consider a location inference attack by the SP, based on Voronoi diagram \cite{voronoiDiagram}, on a cloaked rider if the closest driver is selected.  They give a solution to the attack in which the SP uses a probabilistic model to choose a driver and show that their solution provides a better selection of driver compared to {\em PrivateRide}.
%Duan \etal \cite{Duan2019APO} improve on the work of Khazbak \etal \cite{khazbak} to propose a discount-based solution that provides incentive to riders based on performance decrease in driver selection, while preserving rider privacy.   In their model, drivers upload their exact location to the SP.  
%%B-ride \cite{raza_bride} is a ride-sharing solution that uses a cloaking area for rider, but the pickup location of the drivers are sent to the rider.   
%TIFS Another ride-sharing solution, SRide \cite{sride_ref} aims at preserving rider as well as driver privacy, and is designed for long-distance inter-city ride-sharing travel.   
%\cite{he_ridesharing} is a ride-sharing solution for long-distance travel in which the SP selects a driver whose encrypted pre-defined spatial regions, matches riders whose source and destinations are in those regions.
%TIFS Semenko \etal \cite{semenko_saucez} propose a fully decentralized multi-layered distribution architecture which is completely different from traditional centralized models like that of Uber.  In their model they provide an ``approximate'' location of the drivers, however they do not give more details on how the locations are derived nor any counter-effects of the same.
%In their model, the SP matches the rider and driver using their individual cloaked regions with a weighted bipartite matching algorithm.  Since the matching might not be optimal due to location obfuscation, they propose to incentivise the rider to account for  sub-optimality of driver selection. 
%The work by Al-Momani \etal titled {\em Ride and Hide} \cite{rideandhide} proposes the concept of predefined taxicab stops to hide exact pickup and dropoff points.  This implies an additional overhead of walking on part of the riders to any nearby stop of their choice.  Their work investigates the trade-offs for privacy gains comparing with traditional RHS.
\indent {\em ORide} \cite{ORidePaper} is a follow-up work by the same authors of {\em PrivateRide} that provides more robust privacy and accountability guarantees, and has been described earlier in this paper.  All the following works try to improve upon ORide by proposing different models of privacy-preserving closest driver selection by the SP.  We note here that our attack is relevant in cases where the rider gets to make a choice, and is not applicable in situations where the SP selects a single suitable driver and provides the same to the rider.
{\em pRide} by Luo \etal \cite{pRideLuo} proposes a privacy-preserving ride-matching service involving two non-colluding servers with one being the SP and the other a third-party Crypto Provider (CP).   The solution makes use of Road Network Embedding (RNE) \cite{shahabiRNE} technique to transform a road network into a higher dimensional space so that the distance computation between any two nodes in the network can be performed efficiently.  They propose two solutions, one using the Paillier cryptosystem and another using BGN cryptosystem.  The homomorphically encrypted driver and rider locations received by the SP are sent to the CP along with a random noise where it is decrypted and garbled.  The SP then uses a garbled circuit to find the closest driver to the rider and completes the ride request.  They show high accuracy in matching the closest driver while preserving the privacy of driver and rider locations.   The disadvantage of this scheme is their use of a second Crypto Server that does not collude with the SP, which may be inconvenient to realize in practice, and also the high communication cost between the two servers.   
%Another work named \emph{pRide} by Luo \etal \cite{pRideLuoHWEnclave} makes use of a secure hardware enclave like Intel SGX.  Encrypted location information of drivers and riders are sent to the enclave which first decrypts it and then runs a ride-matching algorithm to return the closest driver to the rider.  In order to prevent leakage of side-channel information they propose data-oblivious algorithms for distance computing and sorting to enhance the security of their scheme.
{\em lpRide} by Yu \etal \cite{lpRideYu} improves upon {\em pRide} to perform all the homomorphic distance computation algorithms on a single SP server thus eliminating high communication cost when two servers are involved.  They use modified Paillier cryptosystem \cite{nabeelPaillier} for encrypting RNE transformed locations of rider and driver.  However, \cite{lpRideAttackSV} proposed an attack on the modified Paillier scheme used in lpRide, allowing the service provider to recover locations of all riders and drivers in the region. 
%While they achieve an efficient privacy-preserving RHS using no external third-party entities, the security of the modified Paillier scheme is not well understood yet and it is uncertain if the security of the modified scheme follows from the hardness of composite residuosity problem as the original Paillier scheme.   
Wang \etal propose {\em TRACE} \cite{wangTrace} that uses bilinear pairing for encrypting driver and rider locations.  {\em PSRide} by Yu \etal \cite{yuPSRIde} uses Paillier cryptosystem and Yao's garbled circuit with two servers on the same lines as {\em pRide} and hence suffers from some of the disadvantages mentioned above.
\textit{EPRide} by Yu \etal \cite{epRideYu} efficiently finds the exact shortest road distance using a road network hypercube embedding. They experimentally show significant improvements in accuracy and efficiency compared to \textit{ORide} and \textit{pRide}. Xie \etal \cite{xieTifs2021} compute shortest distances using road network embeddings along with property-preserving hash functions. In doing so, they remove the need for a trusted third-party server.  \\
\indent Maouche \etal \cite{maouche_attack} propose a user re-identification attack on four different mobility 
datasets obfuscated using three different Location Preserving Privacy Mechanisms (LLPM), with one of the datasets in the RHS setting.   Their attack makes use of previously learned user profiles and tries to re-
associate the same to obfuscated data.
A number of LLPMs are available in the literature that anonymize private data.  
Differential privacy and $k$-anonymity are two popular techniques.  Differential privacy, introduced by the seminal work of Dwork \etal \cite{dwork_diff_privacy} can be applied wherever
aggregate information from several similar entities are available.   
Geo-indistinguishability by Andr\'{e}s \etal \cite{geo_indis}
adds exponentially decaying noise from a Laplace distribution around the point of interest thereby obfuscating the point of interest.  
The notion of $k$-anonymity by Sweeney 
~\cite{sweeny_k_anon} obfuscates an entity by introducing $k-1$ dummy uniformly distributed entities which
are indistinguishable by the adversary.  
In our case, the driver applies noise to her coordinates before encrypting and sending to SP.   SP homomorphically computes the Euclidean distance between the rider and each driver.   
Using this (noisy) Euclidean distance, the rider solves the Gauss circle problem and filters out solutions depending on whether they have a road in their vicinity. Finally, the rider ends up with not one, but many possible choices for the anonymized driver location. This is a combination of both differential privacy (where the driver applies noise to her location) and $k$-anonymity (the rider has many equally possible choices for the driver’s obfuscated location). 
% However, it is also different from differential privacy (since the adversary receives not one but many possible obfuscated locations each time) and k-anonymity (the rider receives a noisy Euclidean distance).
Empirically, we see that our method of adding uniformly random noise is 
sufficient to provide high anonymity to the driver.   Also, our method of filtering out non-plausible
driver locations is based on the region's topography.  We leave
the analysis of using other obfuscation techniques to thwart our attack for future work. 


 
%Kanza \etal propose {\em cryptotransport} \cite{kanzaCryptoTransport}, an RHS solution using cryptocurrency and blockchain while preserving privacy.  In this solution, riders and drivers use pseudonyms to hide their actual identities, where the rider chooses an {\em area}, whose size depends on user-desired privacy, and to hail a ride posts a ledger entry giving her public key, pick-up area and destination area.  From the ledger entry, an interested driver will use the public key to encode her location details and posts a ledger entry upon which the rider will decrypt using her private key to proceed with one-to-one correspondence with driver for ride initiation. 
%We see that there have been many improvements on specific dimensions by each of the works mentioned above.  Currently, computations involving high-depth circuits in a fully homomorphic setting or a multi-party computation setting is not very efficient due to which more work needs to be done in the area of RHS to get a better solution in all the different dimensions.

% Based on the works mentioned above (and prior to the current work), we believe that the solution proposed by ORide is still relevant and useful as a privacy preserving RHS due to the completeness of the solution and ease of deployment and integration with current non-privacy-preserving RHS systems.

